Dual Reader-Parser on Hybrid Textual and Tabular Evidence for Open Domain Question Answering

The current state-of-the-art generative models for open-domain question answering (ODQA) have focused on generating direct answers from unstructured textual information. However, a large amount of world's knowledge is stored in structured databases, and need to be accessed using query languages such as SQL. Furthermore, query languages can answer questions that require complex reasoning, as well as offering full explainability. In this paper, we propose a hybrid framework that takes both textual and tabular evidence as input and generates either direct answers or SQL queries depending on which form could better answer the question. The generated SQL queries can then be executed on the associated databases to obtain the final answers. To the best of our knowledge, this is the first paper that applies Text2SQL to ODQA tasks. Empirically, we demonstrate that on several ODQA datasets, the hybrid methods consistently outperforms the baseline models that only take homogeneous input by a large margin. Specifically we achieve state-of-the-art performance on OpenSQuAD dataset using a T5-base model. In a detailed analysis, we demonstrate that the being able to generate structural SQL queries can always bring gains, especially for those questions that requires complex reasoning.

==> old_experiment.tex <==
\section{Experiments}
In this section, we report the performance of the proposed method on several hybrid open-domain QA datasets.

\subsection{Datasets}\label{ssec:datasets}
We test the proposed method on (1) the mixture of SQuAD-v1.1 \citep{rajpurkar2016squad} and WikiSQL \citep{zhongSeq2SQL2017} datasets and (2) the NaturalQuestions (NQ) \citep{kwiatkowski2019natural} both in the open-domain setting.

\paragraph{Mixture of SQuAD and WikiSQL}
We create a hybrid open QA dataset by mixing SQuAD and WikiSQL data. From now on, we call this mixed dataset \textbf{Mix-SQuWiki}.

\begin{itemize}
    \item SQuAD-v1.1 \citep{rajpurkar2016squad} is a reading comprehension dataset consisting of 100,000+ questions posed by annotators on a set of Wikipedia articles, where the answer to each question is a span from the corresponding paragraph. In the open-domain setting, the passages are retrieved from the Wikidumps on Dec. 21, 2016. We also follow the preprocessing method in \citet{chen2017reading,karpukhin2020dense,izacard2020leveraging} and get passages of 100 words without overlapping.
    
    \item WikiSQL \citep{zhongSeq2SQL2017} is a dataset of 80,654 annotated questions and SQL queries distributed across 24,241 tables from Wikipedia. In this paper, we truncate and serialize each table into passages not exceeding 100 words, respecting row boundaries.
\end{itemize}

\noindent The new dataset Mix-SQuWiki contains all the questions from both SQuAD and WikiSQL datasets, and for each question, we retrieve a set of hybrid candidates from both textual and tabular passages.
 
    
\paragraph{NaturalQuestions}
NaturalQuestions (NQ) \citep{kwiatkowski2019natural} contains questions that are real Google search queries. Similar to \citet{kwiatkowski2019natural}, we only keep questions with short answers for the open-domain setting.

For the textual evidences, we use the Wikipedia dumps on Dec. 20, 2018 for NQ and also truncate the paragraphs into non-overlapping passages of 100 words. To create the tabular evidences, we combine 1.6M Wikipedia tables \citep{bhagavatula2015tabel} and all the WikiSQL tables, and truncate and flatten each table into passages not exceeding 100 words, in the same format mentioned in the previous section.


\paragraph{WikiSQL-both} This dataset is a subset of the WikiSQL data and contains the questions that can be answered by both textual and tabular evidences. We select these questions in a weakly-supervised way by only keeping a question if it has both positive textual and tabular BM25 candidates. For example in Figure \ref{fig:overall_pipeline}, the answer ``Columbia Pictures" can be found in both types of passages. 
% \peng{Maybe you also add a footnote here about how you filter out trivia cases?}



\subsection{Retrieval and Reranking Results}
In this section, we investigate the performance of the BM25 retriever and the BERT reranker using top-k recalls, MAP and MRR as our evaluation metrics.

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[htb]
\centering
% \small
\begin{tabular}{l|cc|cc|c}
\toprule
              & BM25                  & \cellcolor[HTML]{E7FAFE}Reranker         & BM25                  & \cellcolor[HTML]{E7FAFE}Reranker         & \multicolumn{1}{c}{\cellcolor[HTML]{E7F0FE}Reranker}      \\
\textbf{Index} & \textbf{textual}     & \cellcolor[HTML]{E7FAFE}\textbf{textual} & \textbf{tabular}     & \cellcolor[HTML]{E7FAFE}\textbf{tabular} & \multicolumn{1}{c}{\cellcolor[HTML]{E7F0FE}\textbf{hybrid}} \\
\hline
Top-1          & 34.40                & \cellcolor[HTML]{E7FAFE}69.76            & 1.60                 & \cellcolor[HTML]{E7FAFE}10.16            & \cellcolor[HTML]{E7F0FE}69.92                             \\
% Top-2          & 42.40                & \cellcolor[HTML]{E7FAFE}74.40            & 2.52                 & \cellcolor[HTML]{E7FAFE}12.82            & \cellcolor[HTML]{E7F0FE}74.62                             \\
% Top-3          & 46.90                & \cellcolor[HTML]{E7FAFE}76.36            & 3.20                 & \cellcolor[HTML]{E7FAFE}14.84            & \cellcolor[HTML]{E7F0FE}76.74                             \\
% Top-4          & 50.38                & \cellcolor[HTML]{E7FAFE}77.62            & 3.84                 & \cellcolor[HTML]{E7FAFE}15.78            & \cellcolor[HTML]{E7F0FE}78.10                             \\
% Top-5          & 52.58                & \cellcolor[HTML]{E7FAFE}78.42            & 4.22                 & \cellcolor[HTML]{E7FAFE}16.64            & \cellcolor[HTML]{E7F0FE}79.06                             \\
Top-10         & 59.38                & \cellcolor[HTML]{E7FAFE}80.30            & 6.34                 & \cellcolor[HTML]{E7FAFE}18.88            & \cellcolor[HTML]{E7F0FE}80.90                             \\
Top-25         & 65.92                & \cellcolor[HTML]{E7FAFE}81.64            & 8.84                 & \cellcolor[HTML]{E7FAFE}21.20            & \cellcolor[HTML]{E7F0FE}82.42                             \\
Top-50         & 72.16                & \cellcolor[HTML]{E7FAFE}82.50            & 12.36                & \cellcolor[HTML]{E7FAFE}22.62            & \cellcolor[HTML]{E7F0FE}83.26                             \\
Top-100        & 76.50                & \cellcolor[HTML]{E7FAFE}83.44            & 15.04                & \cellcolor[HTML]{E7FAFE}23.72            & \cellcolor[HTML]{E7F0FE}84.10                             \\
% Top-200        & 80.48                & \cellcolor[HTML]{E7FAFE}84.02            & 17.80                & \cellcolor[HTML]{E7FAFE}25.76            & \cellcolor[HTML]{E7F0FE}85.18                             \\
\hline
MAP            & 28.84                & \cellcolor[HTML]{E7FAFE}49.94            & 2.22                 & \cellcolor[HTML]{E7FAFE}7.52             & \cellcolor[HTML]{E7F0FE}46.48                             \\
MRR            & 42.86                & \cellcolor[HTML]{E7FAFE}73.59            & 3.15                 & \cellcolor[HTML]{E7FAFE}13.09            & \cellcolor[HTML]{E7F0FE}73.90                             \\
\bottomrule

\end{tabular}
\caption{\label{tab:recall_squad}Recalls on top-$k$ textual, tabular or the hybrid candidates for SQuAD questions.}
\end{table*}


During both training and inference, for each question, the textual and tabular passages are reranked jointly using a single reranker. On the Mix-SQuWiki dataset, we report the reranking results on SQuAD questions in Table \ref{tab:recall_squad}. The result on WikiSQL questions is in Table \ref{tab:recall_wikisql} in Appendix. To provide better insights on the reranker's performance, we show the top-$k$ recalls on textual, tabular and hybrid evidences separately.
% \peng{How many candidates are reranked in each of three cases during inference?}

From Table \ref{tab:recall_squad}, on both textual and tabular candidates, recall@25 of the ranker is even higher than recall@200 of the BM25 retriever. This suggest that during inference, instead of providing 200 BM25 candidates to the fusion-in-decoder (FID), 25 reranked candidates suffice. 
% Fewer candidates could help save memories and hence speed up the inference\peng{Speeding up inference is questionable because you need to count the time of reranking}. 
In Table \ref{tab:recall_wikisql} and \ref{tab:recall_nq} in Appendix, we observe similar trend with top-25 recalls comparable to top-100 recalls. And in all tables, the recalls on hybrid inputs are almost the same as or even better than the best recalls on individual textual or tabular inputs, meaning that the reranker is able to jointly rank both types of candidates and provide better evidences to the next component -- the reader-parser.
% For example, in Table \ref{tab:recall_nq}, the recall for the top-25 hybrid candidates is 80.03\%, which is higher than the recall for top-25 textual candidates (78.42\%) and top-25 tabular candidates (42.24\%).
% This also indicates that our joint reranker indeed can combine both textual and tabular candidates together to provide better evidences to answer the questions.

\subsection{Performance of the Reader-Parser}
In this section, we discuss the performance of the dual reader-parser.

\paragraph{Evaluation} We report the following metrics on our predictions.
\begin{itemize}
    \item For the baseline models, we report the standard exact match metric (EM) and F1 scores \citep{rajpurkar2016squad} on the predicted answers, using the official evaluation script for SQuAD-v1.1.
    \item For the baseline models, we report both execution accuracy and logical form accuracy \citep{zhongSeq2SQL2017} on the predicted SQL queries, using the official evaluation script.
    \item For all the models, we report an additional metric called \textbf{Top-1-EM}. To calculate this new metric, if the top-1 generated output (using beam search) is a SQL query, we execute the query and get the final answer (if the query is not executable, then we automatically count the answer as wrong). Then we just calculate the EM score on all the top-1 answers.
    \item \textbf{Executable SQLs} stands for the percentage of generated SQLs that are executable. \textbf{\% Direct Ans in Top-1} represents the percentage of top-1 generations that are direct answers, and \textbf{\% SQL in Top-1} is the percentage of top-1 generations that are SQL queries.
\end{itemize}

\paragraph{Technical Details}
Similar to \cite{izacard2020leveraging}, we initialize the fusion-in-decoders with the pretrained T5 model \citep{raffel2019exploring}, and in this paper, we only explore using T5-base model, which has 220M parameters. We use the Adam optimizer \citep{kingma2014adam} with a maximum learning rate of $10^{-4}$ and a dropout rate of 10\%. The learning rate linearly warms up to $10^{-4}$ and then linearly anneals to zero. We train the model for 10k gradient steps with a batch size of 64, and save a checkpoint every 1k steps. When there are multiple answers for one question, we randomly sample one answer from the list. Unless otherwise specified, in the single-type input setting, the candidates are either 50 textual passages or 50 tables, while in the hybrid setting, the input consists of 50 hybrid candidates. During training, the candidates are from BM25 and for each question, we randomly sample one positive candidate and $k$ ($k=24$ for single-type input and $k=49$ for hybrid input) negative candidates from the BM25 results. During inference, the candidates are reranked by the hybrid reranker, to guarantee higher recalls. We generate answers using beam search with beam size 3.

\subsubsection{Model Types}
We first describe different models we used in the experiments. These model all have the same fusion-in-decoder structure but trained on different data.

\paragraph{Baseline Models}
The baseline models are trained using single-type evidences.
\begin{itemize}
    \item \textbf{s-tex} and \textbf{w-tab}: The \textbf{s-tex} model is trained on SQuAD questions with textual evidences (the regular open SQuAD setting), and the \textbf{w-tab} model is trained on WikiSQL questions with tabular evidences.
    % These two models demonstrate how well the fusion-in-decoder performs on single-type inputs, and can be comparable to state-of-the-art results on each dataset.
    \item \textbf{sw-tex} and \textbf{sw-tab}: The model \textbf{sw-tex} is trained on all Mix-SQuWiki questions with textual evidences, and the model \textbf{sw-tab} is trained on all Mix-SQuWiki questions with tabular evidences.
    % \item All the \textbf{*-tex} models are trained to generate textual answers and the \textbf{*-tab} models learn to generate both textual answers and SQL queries.
\end{itemize}
All the \textbf{*-tex} models are trained to generate textual answers and the \textbf{*-tab} models learn to generate both textual answers and SQL queries.

\paragraph{Hybrid Models}
The hybrid models take both textual and tabular evidences as input.
\begin{itemize}
    \item \textsc{DuRePa}: This is a full hybrid model trained on all Mix-SQuWiki questions with hybrid evidences, and generates both answers and SQL queries.
    \item \textsc{DuRePa--}: For comparison, we also train another hybrid model that reads hybrid candidates but only learns to generate direct answers. This is in order to investigate whether learning to generate SQL queries is helpful.
\end{itemize}

%NOTE to Henry: check the following part later.

\begin{table*}[!htb]
\centering
\begin{tabular}{clccccccc}
\toprule
\textbf{Question} & \textbf{Model} &  \textbf{Candidate} & \textbf{Exe}           & \textbf{LF}            & \textbf{Top-1}    & \textbf{EM}                & \textbf{F1}                &  \\
\textbf{type} &  &  \textbf{type} & \textbf{accuracy} & \textbf{accuracy} & \textbf{EM} &&&  \\
\hline
SQuAD & s-tex &  textual                 & \multicolumn{1}{c}{-}      & \multicolumn{1}{c}{-}      & \multicolumn{1}{c}{56.4} & \multicolumn{1}{c}{56.4}       & \multicolumn{1}{c}{66.9}       &  \\
SQuAD & \textsc{DuRePa} &  hybrid                 & \multicolumn{1}{c}{5.1}       & \multicolumn{1}{c}{-}       & \multicolumn{1}{c}{57.0} & \multicolumn{1}{c}{57.0} & \multicolumn{1}{c}{66.7} &  \\
\hline
SQuAD & FID-base & textual (100) & - & - & - & 53.4 & - \\
SQuAD & FID-large & textual (100) & - & - & - & 56.7 & - \\
SQuAD & MP & - & - & - & - & 53.0 & 60.9 \\
SQuAD & PR & - & - & - & - & 56.5 & 63.8 \\
\hline
\hline
WikiSQL                & w-tab &  tabular               & \multicolumn{1}{c}{40.2}       & \multicolumn{1}{c}{61.5}       & \multicolumn{1}{c}{40.2} & \multicolumn{1}{c}{-}      & \multicolumn{1}{c}{-}      &   \\
WikiSQL                & \textsc{DuRePa} &  hybrid                & \multicolumn{1}{c}{38.8} & \multicolumn{1}{c}{59.7} & \multicolumn{1}{c}{42.6} & \multicolumn{1}{c}{34.0} & \multicolumn{1}{c}{37.7} &  \\
\bottomrule
\end{tabular}
\caption{\label{tab:compare-to-baseline}Performance of the baseline and hybrid models. We also compare the results to Multi-Passage BERT (MP) \citep{wang2019multi}, Path Retriever (PR) \citep{asai2019learning} and FID \citep{izacard2020leveraging}.}
\end{table*}

\subsubsection{Comparison to Baseline Models}


In Table \ref{tab:compare-to-baseline}, we compare the hybrid model with the baseline models on SQuAD and WikiSQL questions separately. On the SQuAD questions, the baseline model \textbf{s-tex} achieves EM score of 56.4 using only 50 reranked passages, higher than the EM score of 53.4 by FID-base \citep{izacard2020leveraging} using 100 passages. Using hybrid evidences, the model \textsc{DuRePa} attains a slightly higher EM of 57.0, which beats the FID-large result from \citet{izacard2020leveraging}. These results show that reranking the passages really help boost the end-to-end performance. 

On the WikiSQL questions, the baseline model achieves 40.2 execution accuracy and 61.5 logical form accuracy, which are actually comparable to the Seq2SQL baseline in \citet{zhongSeq2SQL2017}. The current state-of-the-art that is not execution-guided is from \citet{lyu2020hybrid} where the execution accuracy is 89.1 and logical form accuracy is 83.6. But their setting is closed-domain where each question is given the corresponding table, while we need to find evidences from more than 20k tables. Our hybrid model achieves slight lower execution and logical form accuracy, but still beat the baseline on top-1 EM. This might be because it is easier to answer some WikiSQL questions by using textual evidences. In fact, the EM score on generated direct answers is 34.0, which is close to the 38.8 execution accuracy on the generated SQL queries. We also observe that the logical form accuracy is much higher than the execution accuracy by 20\%, meaning that at least 20\% execution errors are because the model generates the wrong table IDs.



\subsubsection{Results on Mix-SQuWiki questions}

\begin{table*}[!htb]
\centering
\begin{tabular}{cccccc}
\toprule
\textbf{Model} & \textbf{Candidate}        & \textbf{Top-1}                 & \textbf{Executable}    & \textbf{\% Direct Ans} & \textbf{\% SQL}\\
& \textbf{type}  & \textbf{EM} & \textbf{SQLs} & \textbf{in Top-1} &  \textbf{in Top-1} \\
\hline
sw-tex                & textual                      & \multicolumn{1}{c}{34.0}       & \multicolumn{1}{c}{-}   & 100\%  & 0\% \\
sw-tab              & tabular                       & \multicolumn{1}{c}{20.4}     & \multicolumn{1}{c}{88.8\%}        &  48.2\% & 51.8\% \\
% \hline
% sw-tex                & hybrid                      & \multicolumn{1}{c}{}       & \multicolumn{1}{c}{-}   &   &  \\
% sw-tab                & hybrid                       & \multicolumn{1}{c}{}     & \multicolumn{1}{c}{}        &   &  \\
\hline
\hline
\textsc{DuRePa}--                & hybrid                      & \multicolumn{1}{c}{40.0}       & \multicolumn{1}{c}{-}   &  100\% & 0\% \\
% \hline
% sw                 & textual                      & \multicolumn{1}{c}{34.8}       & \multicolumn{1}{c}{0.0\%}       & 97.4\%  & 2.6\% \\
% sw               & tabular                       & \multicolumn{1}{c}{22.3}     & \multicolumn{1}{c}{61.7\%}        &  45.7\% & 54.3\% \\
\hline
\textsc{DuRePa}                & hybrid                     & \multicolumn{1}{c}{\textbf{47.9}} & \multicolumn{1}{c}{88.6\%}       &  66.5\%     & 33.5\% \\
\bottomrule
\end{tabular}
\caption{\label{tab:main_result}Results on all Mix-SQuWiki questions.}
\end{table*}

In this subsection, we compare the model performance on all the Mix-SQuWiki questions. Some of these questions can only be answered by passages while some others can only be answered by tables. The results are summarized in Table \ref{tab:main_result}.

First of all, if we only use a single type of evidence, the best top-1 EM is 34.0 achieved by the model \textbf{sw-tex} using textual candidates. However, if we make use of hybrid evidences, the hybrid model \textsc{DuRePa} attains a significantly better top-1 EM of 47.9. It indicates that both textual and tabular evidences are required to answer all the questions from Mix-SQuWiki.

Furthermore, we observe that the model \textsc{DuRePa} has better top-1 EM compared to \textsc{DuRePa--}, suggesting that the answers for some of these questions are not extractive, and need to be obtained by executing SQL queries. In Table \ref{tab:squwiki}, we sampled some questions on which the model \textsc{DuRePa} predicts the correct answers but the model \textsc{DuRePa--} fails. 



\subsubsection{Results on WikiSQL-both Questions}

\begin{table*}[!htb]
\centering
\begin{tabular}{ccccccc}
\toprule
\textbf{Model} &  \textbf{Candidate}        & \textbf{Top-1}                 & \textbf{Executable}    & \textbf{\% Direct Ans} & \textbf{\% SQL}\\
& \textbf{type} &  \textbf{EM} & \textbf{SQLs} & \textbf{in Top-1} &  \textbf{in Top-1} \\
\hline
sw-tex                  & textual                      & \multicolumn{1}{c}{38.7}       & \multicolumn{1}{c}{-}  &  100\% & 0\% \\
sw-tab                & tabular                       & \multicolumn{1}{c}{46.9}     & \multicolumn{1}{c}{86.6\%}        & 60.4\%  & 39.6\% \\
\hline
% sw                   & textual                 & \multicolumn{1}{c}{0.4684}      & \multicolumn{1}{c}{0.00\%}       & 98.69\% & 1.31\%  \\
% sw                    & tabular                  & \multicolumn{1}{c}{0.6016}      & \multicolumn{1}{c}{83.39\%}       & 69.66\% & 30.34\%   \\
\hline
\textsc{DuRePa}--                & hybrid                       & \multicolumn{1}{c}{43.2}     & \multicolumn{1}{c}{-}        &  100\% & 0\% \\
\hline
\textsc{DuRePa}                & hybrid                     & \multicolumn{1}{c}{\textbf{52.7}}       & \multicolumn{1}{c}{86.5\%}   & 60.2\% & 39.8\%  \\
\bottomrule
\end{tabular}
\caption{\label{tab:wikisql-both}Results on WikiSQL-both questions, which are WikiSQL questions that can be answered by both textual and tabular evidences.}
\end{table*}

\begin{table*}[!htb]
\centering
\begin{tabular}{ccccccc}
\toprule
\textbf{Model}  & \textbf{Candidate}        & \textbf{Top-1}                 & \textbf{Executable}    & \textbf{\% Direct Ans} & \textbf{\% SQL}\\
& \textbf{type} & \textbf{EM} & \textbf{SQLs} & \textbf{in Top-1} &  \textbf{in Top-1} \\
\hline
sw-tex              & textual                      & \multicolumn{1}{c}{\textbf{22.0}}       & \multicolumn{1}{c}{-}       &  100\% & 0\% \\
sw-tab           & tabular                       & \multicolumn{1}{c}{5.6}     & \multicolumn{1}{c}{25.8\%}        & 58.2\%  & 41.8\% \\
% \hline
% sw                   & textual                 & \multicolumn{1}{c}{19.9}      & \multicolumn{1}{c}{0.0\%}       & 99.5\% & 0.5\% \\
% sw                 & tabular                  & \multicolumn{1}{c}{5.5}      & \multicolumn{1}{c}{39.7\%}       & 55.7\% & 44.3\%  \\
\hline
\hline
\textsc{DuRePa}--                & hybrid                     & \multicolumn{1}{c}{20.0}       & \multicolumn{1}{c}{-}   & 100\% & 0\% \\
\hline
\textsc{DuRePa}                & hybrid                     & \multicolumn{1}{c}{20.3}       & \multicolumn{1}{c}{53.2\%}   & 77.1\% & 22.9\% \\
\bottomrule
\end{tabular}
\caption{\label{tab:zero-shot-nq}Zero-shot learning: we directly test the generative model trained on Mix-SQuWiki data on the open NQ questions.}
\end{table*}

In the previous subsection, we investigate the situation when some questions can only be answered by either textual or tabular evidence. In this section, we study the questions in the WikiSQL-both dataset. All these questions can be answered by both types of evidences. The purpose of this experiment is to study when both textual and tabular evidences are plausible, whether the model can pick one answers a question better.

From Table \ref{tab:wikisql-both}, first of all, the sw-tab model using tabular evidences behaves better than the sw-tex model using textual evidences. It means even when both evidences provide the answer, the difficulties in using the evidences are different. On WikiSQL questions, using tabular information leads to better answers.

Secondly, when using only one type of evidence, the sw-tex and sw-tab models behave significantly worse than the hybrid model. This indicates that the hybrid model can again figure out which evidence type should be used to provide the correct final answer.


\subsubsection{Zero-shot Learning on NQ Questions}




Finally, we study the zero-shot learning performance of the models on the open NQ questions. Since we include extra 1.6M Wikipedia tables \citep{bhagavatula2015tabel}, the models need to deal with not only unseen questions, but also unseen evidences. Therefore, it is challenging for the models to generate correct answers and even more challenging to obtain the answers by SQL queries.

From Table \ref{tab:zero-shot-nq}, we observe that the model \textbf{sw-tex} achieves the highest top-1 EM score, followed by the hybrid model \textsc{DuRePa}. We also observe that 53.2\% of the generated SQLs are actually executable. But through some error analysis, most of these executable SQLs return empty lists. It means the generated SQLs have correct column names, but the generated cell values cannot be found in the predicted tables. We illustrate some such errors in Table \ref{tab:nq_errors}, and also provide some correctly predicted examples in \ref{tab:nq_examples}.


% \begin{table*}[htb]
% \centering
% \begin{tabular}{clllrrr}
% \toprule
% \textbf{Model} & \textbf{Question} & \textbf{Candidate}        & \textbf{Top-1}                 & \textbf{Executable}    & \textbf{\% Direct Ans} & \textbf{\% SQL}\\
% & \textbf{type} & \textbf{type} & \textbf{EM} & \textbf{SQLs} & \textbf{in Top-1} &  \textbf{in Top-1} \\
% \hline
% nq-tex & NQ              & textual                      & \multicolumn{1}{c}{}       & \multicolumn{1}{c}{}       &   &  \\
% nq-tab & NQ           & tabular                       & \multicolumn{1}{c}{}     & \multicolumn{1}{c}{}        &   &  \\
% \hline
% nq & NQ                  & textual                 & \multicolumn{1}{c}{0.4559}      & \multicolumn{1}{c}{-}       & 100\% & 0\% \\
% nq & NQ                  & tabular                  & \multicolumn{1}{c}{0.1527}      & \multicolumn{1}{c}{-}       & 100\% & 0\%  \\
% \hline
% nq & NQ               & hybrid                     & \multicolumn{1}{c}{\textbf{0.4628}}       & \multicolumn{1}{c}{-}   & 100\% & 0\% \\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:nq}NQ}
% \end{table*}


\begin{table*}[!htb]
\centering
\small
\begin{tabularx}{\textwidth}{lX}
\toprule
% \multicolumn{2}{1}{Examples of the SQuWiki questions that are answered correctly by model DUREPA but incorrectly bymodel }
% \midrule

\textit{\textbf{Question:}}                & Which party won in the election in voting district Kentucky 5?                                                                                                     \\
\textit{\textbf{Groundtruth:}}             & {[}'democratic'{]}                                                                                                                                                 \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}:}}  & \texttt{sql: SELECT Party FROM table\_1-1342218-17 WHERE District = "Kentucky 5"}                                                                                           \\
\textit{\textbf{Execution result:}}        & {[}'democratic'{]}                                                                                                                                                 \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}--}} & answer: republican                                                                                                                                                 \\
% \hline
% \textit{\textbf{Question:}}                & What was the control for the year with a Conservative Party result of 10 (+5)?                                                                                     \\
% \textit{\textbf{Groundtruth:}}             & {[}'labour hold'{]}                                                                                                                                                \\
% \textit{\textbf{Top-1 generation by sw:}}  & \texttt{sql: SELECT Control FROM table\_2-16041438-1 WHERE Conservative Party = "10 (+5)"}                                                                                  \\
% \textit{\textbf{Execution result:}}        & {[}'labour hold'{]}                                                                                                                                                \\
% \textit{\textbf{Top-1 generation by sw--}} & answer: no overall control                                                                                                                                         \\
%                                           &                                                                                                                                                                    \\
\hline
\textit{\textbf{Question:}}                & Which Condition has an unaffected Partial thromboplastin time, Platelet count, and a Prothrombin time?                                                             \\
\textit{\textbf{Groundtruth:}}             & {[}'aspirin', 'uremia', "glanzmann's thrombasthenia"{]}                                                                                                            \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}:}}  & \texttt{sql: SELECT Condition FROM table\_1-14006-1 WHERE Partial thromboplastin time = "Unaffected" AND Platelet count = "Unaffected" AND Prothrombin time = "Unaffected"} \\
\textit{\textbf{Execution result:}}        & {[}'uremia', "glanzmann's thrombasthenia", 'aspirin'{]}                                                                                                            \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}--}} & answer: vitamin k deficiency or warfarin                                                                                                                           \\
% \hline
% \textit{\textbf{Question:}}                & What was the date that the decision was Niittymaki, the attendance larger than 19,207, and the record 28–17–5?                                                     \\
% \textit{\textbf{Groundtruth:}}             & {[}'january 31'{]}                                                                                                                                                 \\
% \textit{\textbf{Top-1 generation by sw:}}  & \texttt{sql: SELECT Date FROM table\_2-11902580-6 WHERE Decision = "niittymaki" AND Attendance \textgreater "19,207" AND Record = "28-17-5"}                                \\
% \textit{\textbf{Execution result:}}        & {[}'january 31'{]}                                                                                                                                                 \\
% \textit{\textbf{Top-1 generation by sw--}} & answer: february 31                                                                                                                                                \\
%                                           &                                                                                                                                                                    \\
\hline
\textit{\textbf{Question:}}                & What is the total amount of gold medals when there were more than 20 silvers and there were 135 bronze medals?                                                     \\
\textit{\textbf{Groundtruth:}}             & {[}'1'{]}                                                                                                                                                          \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}:}}  & \texttt{sql: SELECT COUNT(Gold) FROM table\_2-15428689-2 WHERE Silver \textgreater 20 AND Bronze \textgreater 135}                                                          \\
\textit{\textbf{Execution result:}}        & {[}1{]}                                                                                                                                                            \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}--}} & answer: 0                                                                                                                                                          \\
\bottomrule
\end{tabularx}
\caption{\label{tab:squwiki}Examples of the SQuWiki questions that are answered correctly by model \textsc{DuRePa} but incorrectly by model \textsc{DuRePa--}.}
\end{table*}




\begin{table*}[!htb]
\centering
\small
\begin{tabularx}{\textwidth}{lX}
\toprule
\textit{\textbf{Question:}}                & when did amnesia the dark descent come out                                                                                                    \\
\textit{\textbf{Groundtruth:}}             & {[}'8 September 2010'{]}                                                                                                                                                 \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}:}}  & \texttt{sql: SELECT Release Year FROM table\_30576767-1 WHERE Title = \"amnesia: the dark descent\"}                                                                                           \\
\textit{\textbf{Execution result:}}        & {[}{]}                                                                                                                                                 \\
\hline
\textit{\textbf{Question:}}                & how many episodes are there in dragon ball z                                                                                              \\
\textit{\textbf{Groundtruth:}}             & {[}"291 episodes", "291"{]}                                                                                                                                                 \\
\textit{\textbf{Top-1 generation by \textsc{DuRePa}:}}  & \texttt{sql: SELECT COUNT(Episodes) FROM table\_6358299-9 WHERE Title = \"dragon ball z\"}                                                                                           \\
\textit{\textbf{Execution result:}}        & {[}{]}                                                                                                                                                 \\
\hline
\textit{\textbf{Error analysis:}}                  & \textcolor{red}{Both generated SQLs are executable, but returns empty list. It means the generated columns all exist in the tables, but the cell values do not.} \\
\bottomrule
\end{tabularx}
\caption{\label{tab:nq_errors}Examples of erroneous SQL queries on NQ questions.}
\end{table*}




\begin{table*}[!htb]
\centering
\small
\begin{tabularx}{\textwidth}{lX}
\toprule
% \textit{\textbf{Question:}}         & cast of law \& order special victim unit                                                                                                                                                                                                                                                                                                                          \\
% \textit{\textbf{Groundtruth:}}      & {[}'kelli giddish', 'richard belzer', 'stephanie march', 'diane neal', 'ice-t', 'danny pino', 'dann florek', 'tamara tunie', 'michaela mcmanus', 'mariska hargitay', 'adam beach', 'b. d. wong', 'christopher meloni', 'raúl esparza', 'michelle hurd', 'peter scanavino'{]}                                                                                                                                                                                                                                                                                                                                          \\
% \textit{\textbf{Top-1 generation:}} & \texttt{sql: SELECT Cast FROM table\_22266670-7 WHERE Program = "law \& order: special victims unit"}                                                                                                                                                                                                                                                                                      \\
% \textit{\textbf{Execution result:}} & {[}'chris orbach', 'donnetta lavinia grays', 'nicholas gonzalez', 'robert john burke', 'kathryn erbe', 'jerry orbach', 'joel de la fuente', 'john schuck', 'william h. burns', 'dean winters', 'connie nielsen', 'adam beach', 'adam baldwin', 'jesse l. martin'{]}                                                                                                                                                                                                                                                                                                                                           \\
% \multicolumn{2}{l}{\textit{\textbf{}}}    \\
% \hline

\textit{\textbf{Question:}}         & who sings the pokemon theme song season 1                                                                                                                                                                                                                                                                                                                           \\
\textit{\textbf{Groundtruth:}}      & answer: jason paige                                                                                                                                                                                                                                                                                                                                                 \\
\textit{\textbf{Top-1 generation:}} & \texttt{sql: SELECT Vocalist FROM table\_2144389-13 WHERE Title = "pokémon theme" AND Episodes used 1 = "pokémon theme"}                                                                                                                                                                                                                                                     \\
\textit{\textbf{Execution result:}} & {[}'jason paige'{]}                                                                                                                                                                                                                                                                                                                                                 \\
\hline
\textit{\textbf{Question:}}         & when did david akers kick the 63 yard field goal                                                                                                                                                                                                                                                                                                                    \\
\textit{\textbf{Groundtruth:}}      & answer: september 9, 2012                                                                                                                                                                                                                                                                                                                                           \\
\textit{\textbf{Top-1 generation:}} & \texttt{sql: SELECT Date FROM table\_8378967-1 WHERE Distance = "63 yards" AND Kicker = "david akers"}                                                                                                                                                                                                                                                                       \\
\textit{\textbf{Execution result:}} & {[}'september 9, 2012'{]}                                                                                                                                                                                                                                                                                                                                           \\
\hline
\textit{\textbf{Question:}}         & what album is sacrifice by elton john on                                                                                                                                                                                                                                                                                                                            \\
\textit{\textbf{Groundtruth:}}      & answer: sleeping with the past.                                                                                                                                                                                                                                                                                                                                     \\
\textit{\textbf{Top-1 generation:}} & \texttt{sql: SELECT Album FROM table\_4105885-1 WHERE Artist = "elton john" AND Song = "sacrifice"}                                                                                                                                                                                                                                                                          \\
\textit{\textbf{Execution result:}} & {[}'sleeping with the past'{]}                                                                                                                                                                                                                                                                                                                                      \\
\hline
% \textit{\textbf{Question:}}         & who did johnny manziel play college football for                                                                                                                                                                                                                                                                                                                    \\
% \textit{\textbf{Groundtruth:}}      & answer: texas a\&m                                                                                                                                                                                                                                                                                                                                                  \\
% \textit{\textbf{Top-1 generation:}} & sql: SELECT College(s) played for FROM table\_3401335-11 WHERE Player = "johnny manziel"                                                                                                                                                                                                                                                                            \\
% \textit{\textbf{Execution result:}} & {[}'montana', 'ucla', 'texas a\&m', 'california', 'baylor', 'purdue', 'clemson', 'michigan', 'southern california', 'princeton', 'california lutheran', 'cornell', 'oregon', 'columbia', 'yale , rutgers', 'trinity college', 'tennessee', 'texas', 'iowa', 'kentucky state', 'army', 'ohio state', 'mississippi', 'lsu', 'penn state', 'boston college', 'yale'{]} \\
% \multicolumn{2}{l}{\textit{\textbf{}}}                                                                                                                                                                                                                                                                                                                                                                    \\
% \hline
% \textit{\textbf{Question:}}         & who is the original singer of you re going to love me                                                                                                                                                                                                                                                                                                               \\
% \textit{\textbf{Groundtruth:}}      & answer: jennifer holliday                                                                                                                                                                                                                                                                                                                                           \\
% \textit{\textbf{Top-1 generation:}} & \texttt{sql: SELECT Original artist FROM table\_30996994-1 WHERE Song (original artist) = "you re going to love me"}                                                                                                                                                                                                                                                         \\
% \textit{\textbf{Execution result:}} & {[}'whitney houston', 'diana ross', 'dreamgirls', 'blu cantrell', 'the beatles', 'faith hill', 'jennifer holliday', 'monica'{]}                                                                                                                                                                                                                                     \\
% \multicolumn{2}{l}{\textit{\textbf{}}}                                                                                                                                                                                                                                                                                                                                                                    \\
% \hline
% \textit{\textbf{Question:}}         & who wrote the song what child is this                                                                                                                                                                                                                                                                                                                               \\
% \textit{\textbf{Groundtruth:}}      & answer: william chatterton dix                                                                                                                                                                                                                                                                                                                                      \\
% \textit{\textbf{Top-1 generation:}} & \texttt{sql: SELECT Author FROM table\_36169771-1 WHERE Song = "what child is this?"}                                                                                                                                                                                                                                                                                        \\
% \textit{\textbf{Execution result:}} & {[}'william chatterton dix'{]}                                                                                                                                                                                                                                                                                                                                      \\
% \multicolumn{2}{l}{\textit{\textbf{}}}                                                                                                                                                                                                                                                                                                                                                                    \\
% \hline
\textit{\textbf{Question:}}         & who played raquel in only fools and horses                                                                                                                                                                                                                                                                                                                          \\
\textit{\textbf{Groundtruth:}}      & answer: tessa peake-jones                                                                                                                                                                                                                                                                                                                                           \\
\textit{\textbf{Top-1 generation:}} & \texttt{sql: SELECT Actor FROM table\_6994109-1 WHERE Role = "raquel" AND Film/Show = "only fools and horses"}                                                                                                                                                                                                                                                               \\
\textit{\textbf{Execution result:}} & {[}'tessa peake-jones'{]}                                                                                         \\
\bottomrule
\end{tabularx}
\caption{\label{tab:nq_examples}Some predictions under zero-shot learning. These are some correct answers to the NQ questions where the top-1 generation is a SQL query.}
\end{table*}

% \section*{Acknowledgments}

% The acknowledgments should go immediately before the references. Do not number the acknowledgments section.
% Do not include this section when submitting your paper for review.
